Identity Preserve Transform: Understand What Activity Classification Models Have Learnt

Activity classification has observed great success recently. The performance on small dataset is almost saturated and people are moving towards larger datasets. What leads to the performance gain on the model and what the model has learnt? In this paper we propose identity preserve transform (IPT) to study this problem. IPT manipulates the nuisance factors (background, viewpoint, etc.) of the data while keeping those factors related to the task (human motion) unchanged. To our surprise, we found popular models are using highly correlated information (background, object) to achieve high classification accuracy, rather than using the essential information (human motion). This can explain why an activity classification model usually fails to generalize to datasets it is not trained on. We implement IPT in two forms, i.e. image-space transform and 3D transform, using synthetic images. The tool will be made open-source to help study model and dataset design.

==> 0_concept.tex <==
Equation, Eq.~\ref{eq:equation_name}.
Figure, Fig.~\ref{fig:figure_name}.
Table, Tab.~\ref{tab:table_name}.
Section, Sec.~\ref{sec:section_name}.

Put \label{tab:table_name} inside the \caption{} command, or \section{} command.

cite, ~\cite{}

~ is for adding space.

If there are multiple, use \cite{a}\cite{b}, not \cite{a,b}.

Math symbols? How you are picking the math symbol for now? set, vector.

1. Fig, Table, Equation, 

citation.

term confusion.

Priority:

1. label for figure, table, equation.
2. red text, which you know how to modify.
3. main message and introduction.
4. equation

- scheme
- method

==> 1_intro_note.tex <==
Image transform: the identity is the same, no damage to the human motion, background information is preserved as well. TSN performance drop, sometimes it drop a lot, gaussian, 25\%, rotation 25\%. Sensitive to data augmentation.

Semantic transform: $CR_f$, $CR_b$, three distint categories, background is sufficient. object related categories. 
TSN detect activity by detecting correlated object in the image, it can be in the foreground or in the background / environment signal. not using motion and pose. image classification - video classification.
Foreground only - high performance, background only - high performance. 
TSN is not using the pose.

Semantic transform: semantic transform split image into foreground and background. TSN shows three distint clusters of activity. One relies on foreground, one relies on background, one relies on mixture. This can infer TSN is not successfully using the pose information, but rather using patterns in the foreground and background.

3D transform: study the manifold. deeper investigation. Adapt from synthetic to real.
A lot of activity from synthetic data. Viewpoint three factors. The performance is not invariant. Furthermore, human appearance has impact on performance. Consistent weakness for synthetic models, these can be verified with real data as well.

3D transform: Deep investigation of the manifold by control all factors. Model sensitive to viewpoint and appearance. The sensitivity is activity dependent. Some trends are invariant to appearance and can generalize to real world appearance. This unveils the characteristic of the model. Control one factor and randomize all the rest. The conclusion is also valid for the real data.
% viewpoint is well known.
% how to scale up?


==> figure/backup/1_intro_v1.tex <==
\section{Introduction}

Understanding a model is an important topic.

Computer vision models are known to be overfit.

In this paper we study state-of-art models, what they used to make decisions. Whether they are using essential information e.g. human pose, or superficial information.

\cite{zhuotun} shows the vision model can make reliable decision using background information. \cite{iclr_oral} shows vision model makes decision using the texture.

Understanding an activity model is more important than object based task. Activity model has more objects involved, which is combinatory larger. Activity data is much rare and difficult to collect. This makes it easier to overfit. A typical example is a blue pickup doing U-turn. If the dataset is not diverse enough, the model can easily predict the U-turn behavior by blue pickup.

In order to understand the generalization of a model, we propose identity preserving transform (IPT). In the 2D image space, the IPT can be data augmentation or semantic transformation. In the 3D space, the IPT can be viewpoint, lighting, cloth, etc.

This understanding makes us think how to better design an activity classification benchmark.

This paper has following contributions. First, we apply identity perseving transformations to activity classification model to study the generalization of these models. Second, we build a synthetic human activity dataset to benchmark algorithms.

==> figure/backup/1_intro_v2.tex <==
Understanding model is an important topic in computer vision. The thriving of convolutional neural networks (CNNs) and deep learning methods have boost up video activity classification models’ performance, whereas explanations for their high performances remain few. In order to investigate what a trained activity classification model has learnt and whether it can learn the essential information of an activity identity, we propose a scheme called Identity Preserve Transform to answer these questions. With the scheme we study an activity classfication model’s learning ability from the perspective of input data instead of the model architecture, it means that the model keeps its original architecture through out the investgation process. Therefore our approach is suitable for a wide range of video activity classification models, including those not built on CNNs.

A video expressing a human activity can be produced through the following steps: Position the main person in 3-dimensinal space, the person has certain mesh and apperance while doing a symbolic motion. Surround the main person with background which includes scene, lighting, and activity related objects. Select a viewpoint that allows seeing the main person. Record an activity video with a camera. We could abstract 5 information sources from this production process:
Human Motion, Human Appearance ( Mesh \& Texture ), Background ( Scene, Lighting \& Object ), Viewpoint, Camera Recording.

We state that human motion is the most essential information source for human activity identification, which we refer to as human activity identity. However, in practice it is very difficult to extract and represent human motion without the represence of other information sources. On the contrary, Identity Preserve Transform alters the other four information sources to reveal their effects on model performance while keeping human motion consistent, as shown in Fig.~\ref{fig:transform}. 

In Sec.~\ref{sec:method} we demonstrate how Identity Preserve Transform alters each information source and analyze the possible responses given by an activity classification model. This scheme is then applied to state-of-the-art activity classification models built on CNNs to display what they have learnt after training in the Experiments section. Finally, we summarize the insights into activity classification models given by Identity Preserve Transform.

==> figure/backup/2_related_v1.tex <==
\section{Related Work}

% Methods we studied?

The main contribution is about identity preserving transform. Adversarial attack~\cite{}, small perturb. 

Build large scale controllable data 

Synthetic human dataset and dataset for diagnosis.

% Related datasets?

Existing models can achieve great performance on small datasets, such as UCF101~\cite{}. 

% Model understanding and understanding with synthetic data

Computer graphics data is a powerful tool for understanding model behavior. Sintel~\cite{sintel}, Computer graphics imaginary~\cite{}, UnrealStereo~\cite{zhang2018unrealstereo}.

Network dissection, Bolei Zhou. \cite{bau2017network}.

Studies have proven the network fit to background area of images.

Image editing has been widely used \cite{elephant in the room}. \cite{zhu2016object}.

Domain adaptation is a popular topic for using synthetic data. This challenge also exist between different real datasets.~\cite{}.

Use CAM to focus model?

The model can dataset we studied are \cite{}\cite{}, they are not related work.

Understanding the representation of a vision model is an important topic. Study the invariance and equivariance? \cite{lenc2015understanding}.

Show the generalization gap between datasets. What metric, how big the gap is, whether the setup is persuasive.

The relationship between number of activities and generalization power?

Visualization techniques. Model understanding.

Object detector emerges from scene.




==> note.tex <==
Concept definition

Identity preserve transform. Why it is novel, compared with previous ones.

How to call these methods, why they are a coherent method? Why they are novel?

Equation notation.

Issue: the details are flat and the structure is not clear.

1. $$ I = G(\theta_1, \theta_2, \theta_3) $$

Identity preserve transform, 10 factors, 1 factor, 9 factors not related. one factor one section.

1. Image transform, I.
2. Semantic transform, f(). prior information. GAN, change cloth.
3. 3D transform, robotic arm, synthetic data.

Action classification, pose.
Object detection, object x,y, category
Classification, category.

image transform: popular image processing techniques for data augmentation.
semantic transform: image transformation which requires prior knowledge, encoded by a computer vision model.
Use GAN change cloth, image segmentation to separate foreground and background. 

3d transform / full transform / complete transform / oracle transform / scene transform / god transform / synthetic transform / factorized transform.

Main messages??? quantitative result?

constructive / reconstructive / generative?

3D transform can be achieved if individual factors can be controlled separately. Previously, people use robotic arm in a lab setting to control viewpoint and lighting. But this usually expensive and hard to setup. Recently, due to the popularity of synthetic data, people are using synthetic data to control factors of an image, such as viewpoint\cite{}, weather condition\cite{}, material property\cite{}.

robotic arm \cite{NORB, USC}, synthetic driving control weather, 3D attack. 

3D -> change viewpoint
synthetic transform -> real.
material, lighting. 



% citations 
Introduction:
cite{better_activity_model}  TSN,TRN,I3D,P3D,S3D,non-local network
cite{generalization_result_from_yi}
cite{biological_motion_example}

Related works
through removal~\cite{}
classification models are built on multi-branch 2-dimensional CNNs (using 2-D kernels)~\cite{} or 3-dimensional CNNs (using 3-D kernels)~\cite{},

Methods
Image and ground truth were captured using unrealcv~\cite{}
CMU Mocap dataset~\cite{}

Experiment
In this section Identity Preserved Transform is applied to the trained Temporal Segment Networks (TSN) introduced in \cite{} and trained Inflated 3D ConvNet (I3D) introduced in \cite{}. One on hand, TSN is the representative of state-of-the-art video classification models that uses 2D convolutional kernels in neural network.  On the other hand, I3D is the pioneer in 3D CNNs, giving rise to many adaptations such as S3D~\cite{}, I3D-GCN~\cite{}, etc.

We adopted TSN parameters trained on UCF101~\cite{} provided by OpenMMLab~\cite{} and I3D parameters trained on Kinetics~\cite{} provided by deepmind~\cite{} publicly on Github. Both models’ parameters are pre-trained on ImageNet, input modality to both models is RGB without optical flow.


==> note/4_exp.tex <==
% x-axis: activities, y-axis: original, ipt-semantic, novel dataset

\section{Experiment}

In this section Identity Preserved Transform is applied to the trained Temporal Segment Networks (TSN) introduced in \cite{} and trained Inflated 3D ConvNet (I3D) introduced in \cite{}. We adopted TSN parameters trained on UCF101~\cite{} provided by OpenMMLab and I3D parameters trained on Kinetics~\cite{} provided by deepmind publicly on Github. Both models’ parameters are pre-trained on ImageNet, input modality to both models is RGB without optical flow.


\subsection{Implementing Image-space Transform}

Tab.~\ref{tab:image_transform} indicates that even though applying image transform preserves human motion information, it will cause a decline in TSN’s classification performance. \textcolor{red}{Different image processing techniques} give rise to different extents of decline. Among the listed augmentation types except the identical transform (keeping video as its original status), Additve Gaussian Noise and Clockwise Rotation caused relatively intense perturbations to TSN’s performance, it means TSN is susceptible to Gaussian noise and rotation of the human figure.


\input{fig_table/fig_image_transform.tex}

\input{fig_table/tab_image_transform.tex}


Tab.~\ref{tab:image_transform} indicates that even though applying image transform preserves human motion information, it will cause a decline in TSN’s classification performance. \textcolor{red}{Different image processing techniques} give rise to different extents of decline. Among the listed augmentation types except the identical transform (keeping video as its original status), Additve Gaussian Noise and Clockwise Rotation caused relatively intense perturbations to TSN’s performance, it means TSN is susceptible to Gaussian noise and rotation of the human figure.

\subsection{Implementing Semantic Transform}

\input{fig_table/fig_semantic_transform.tex}

We sampled \red{100 videos} from each activity class in UCF101 and generated the foreground-only and background-only video pair for them. Next, we obtained the top-1 test accuracy of TSN on 3 input modes (original, foreground-only, background-only) to compute accuracy changing rates $CR_f$ and $CR_b$ using Eq.~\ref{eq:changing_rates} for each class. \red{A complete report of accuracy changing rates for all UCF101 classes is provided in the supplementary material}. \red{Simultaneously, we adapted Class Activation Mapping~\cite{} for TSN, and generated class activation maps corresponding to the class with highest classification score,} which marked out the most salient region in a video from the view of TSN. Accuracy changing rates over all classes in UCF101 can be categorized as follows:

\textcolor{blue}{Where are these numbers? Make a figure to summarize these results}

Accuracy changing rates over all classes in UCF101 can be categorized as follows:

{\textbf{$0 \approx CR_f \ll CR_b \approx 1$:}} It means the model attaches more importance to the human-centric foreground. Examples are Apply Eye Makeup $(CR_f=0.041,CR_b=1)$ and Shaving Beard $(CR_f=0.02, CR_b=0.94)$ in Fig~\ref{fig:semantic_transform}. To recognize these two human activities requires visual attention to faces and hand motions of the person, therefore TSN correctly localizes the vital region for these two classes.

$1 \approx CR_f \gg CR_b \approx 0$ It means the model attaches more importance to background. Examples are Lunges $(CR_f=1,CR_b=0.091)$ and Golf Swing $(CR_f=1,CR_b=0.021)$ in Fig~\ref{fig:semantic_transform}. \red{In these two cases, main shape of the person is preserved in both foreground-only video and background-only video,} giving a cue about the corresponding human motion. Nevertheless, TSN can not correctly recognize them with foreground but successfully recognizes with background. This indicates for these classes, TSN is drawn to some texture or object in the background while ignoring the human motion.

$\left|CR_f- CR_b\right|< 0.5, 0<CR_f<1, 0< CR_b<1$: It means the model attaches importance to both foreground and background, but neither is enough to achieve as high accuracy as the original video. Examples are Fencing $(CR_f=0.735,CR_b=0.776)$ and Body Weight Squats $(CR_f=0.523,CR_b=0.705)$ in Fig~\ref{fig:semantic_transform}. For these two classes, normal human vision can recognize the human activity with either foreground-only video or background-only video, but TSN needs information from both videos to yield high score for the correct class.

Among various types of human activites in UCF101, those activities that human uses object such as playing instrument, yielded interesting results. As shown in Fig~\ref{fig:semantic_transform}, when the object is more preserved in the background, like Playing Piano $(CR_f=0.8,CR_b=0)$ and Archery $(CR_f=0.957,0.064)$, $CR_b$ is lower than $CR_f$. Whereas, when the object is more preserved in the foreground, like Playing Guitar $(CR_f=0.24,CR_b=0.42)$ and Playing Flute $(CR_f=0,CR_b=0.56)$, $CR_b$ is higher than $CR_f$. Simultaneously, class activation maps of these type of activities show that TSN is drawn to the object in the video.

\textcolor{blue}{Number for this? How this is useful? How is it associated to real world applications?}

If a video activity classfication model has learnt human motion corresponding to each class, it should be able to use the frame-by-frame change of human pose to infer the activity class. Though both the foreground-only video and background-only video preserve the human's shape and pose, we got different reactions from TSN. It indicates that the model needs to detect image components correlated with an activity class in order to recognize this activity. The symbolic image components for an activity class can be texture, edges, objects, etc. When they appear more in the foreground, foreground video activates correct classification and $CR_f$ is low; when they appear more in the background, $CR_b$ is low. Therefore, Semantic Transform revealed to us that \red{TSN lacks an effective mechanism to model} and infer human motion for classifying activities. 


\subsection{Implementing 3D Transform}

\subsubsection{Influence of Viewpoint}

\textcolor{blue}{Not able to extract meaningful information}

\textcolor{blue}{Describe the dataset first, avoid writing too long paragraph.}

\textcolor{red}{In order to study how a video activity classification responds to viewpoint change, we collected a 3-D human animation dataset from CMU Graphics Lab Motion Capture Database* and Unreal Engine Marketplace} that covers 22 human activity classes in Kinetics-400 and 11 activity classes in UCF101. 
Next we selected 5 activity classes for TSN and I3D from this synthetic video dataset respectively to generate 3 data splits over each class:
\begin{itemize}
    \item For TSN: Archery, Golf Swing, Baseball Pitch, Jumping Jack, Playing Violin, Push-ups
    \item For I3D: Archery, Climbing Ladder, Dribbling Basketball, Kicking Soccer Ball, Playing Violin
\end{itemize}
	
\blue{Justify the selection}
	
The 5 activity classes chosen for TSN appear in UCF101, while the 5 activity classes chosen for I3D appear in Kinetics-400. These human activities share a common characteristic: the human motion identifying each activity consists symbolic human pose or large body movements, making it possible to be recognized from different viewpoint. Viewpoint factor settings are as belows:
$$Split_{x} = \{ V_i(x) \mid x_{i+1}=x_{i}+\delta, i=1,2,\cdots,360\}$$
When $x$ refers to azimuth angle, $\delta=1$ and $x_1=0$. When $x$ refers to elevation angle, $\delta=0.25$ and $x_1=-30$. When $x$ refers to camera distance, $\delta=1$ and $x_1=100$.


After recording the scores for each activity class given by TSN and I3D, we found in many data splits that despite minor local fluctuations, the classification score varies along a certain trend as the controlled viewpoint factor changes at fixed step. We selected 6 data splits that display obvious trends in the form of score curve in Fig.~\ref{fig:trends}, results for other data splits are provided in the supplementary material. 


\input{fig_table/fig_trends.tex}



\textcolor{red}{We choose azimuth angle for Push-ups class as an example for further discussion.} The Spatial ConvNet inside TSN is based on Inception Network. We extracted features output by the max-pooling layer following \textcolor{red}{the third Inception Module} and features output by Segmental Consensus layer, \textcolor{red}{then generated PCA embeddings of these two intermediate layers' features}, as shown in Fig.~\ref{fig:pca}. From the PCA embeddings we can see that if the factor traverses across its whole value domain, the manifold converges to become a loop. As the layer goes deeper, the manifold is twisted, entangled and becomes locally coarse. After the Segmental Consensus layer, embeddings corresonding to around 0 azimuth value and 180 value are pulled very close to each other, while embeddings corresponding to around 90 azimuth value and 270 value are turned to the other side at feature space. This shape of manifold echoes with the score curve derived from the final output of TSN. It indicates that when the model prefers viewpoint set towards the person doing push-ups with invariance to left-right flipping, and it can easily fail when viewpoint is set towards the person's face or feet. 


\textcolor{blue}{Avoid limiting conclusion to a specific model and a specific category, you can say it is just an example}

In summary, TSN and I3D are sensitive to viewpoint, and the blind viewpoint depends on activity class as well as the model.

\input{fig_table/fig_pca.tex}

\subsubsection{Influence of Human Appearance}

\textcolor{red}{In order to see whether a video activity classification model will have different responses to different human appearances}, we repeated the viewpoint experiments over 8 different human appearances. On one hand, the classifying accuracy of both TSN and I3D on the aggregation of \(Split_{az}\), \(Split_{el}\), \(Split_{dist}\) is influenced by human appearance, Tab.~\ref{tab:appearance} takes Push-ups as an example. Two models show preference for some same human appearances, i.e. \textcolor{red}{Appearance 5 and Appearance 6}. On the other hand, most score curves' shape varies once human appearance in the video split is changed to another. However, there exist cases where the score curves over different appearances given by a model look similar. For example, TSN responds similarly to all of 8 appearances on the azimuth split over Push-ups. As shown in Fig.~\ref{fig:azimuth}, all score curves peak at around 0 and 180 azimuth and reach the lowest at around 90 and 270. We expect this consistency among different synthetic appearances can generalize to real domain. To verify our supposition, we filmed videos of real human doing push-ups from 6 azimuth angles on two appearances and then recorded TSN‘s classification score for each azimuth angle. The results come out in support of our supposition, TSN's response to azimuth angle change in real Push-ups videos is consistent with the trend emerging from synthetic data, as shown in Fig.~\ref{fig:real_verify}.

\red{From the analysis of viewpoint experiment and human appearance experiment,} taking Push-ups azimuth factor as an example for deep discussion, we can see that 3D transform is able to provide us with insights into activity classification models. Since 3D transfom has access to all kinds of elements and factors in a video, it can reveal to us many details on how a controlled factor take effects on a trained model during human activity classification.


\begin{table*}[]
\centering
\begin{tabular}{|c|c|c|c|c|}
\begin{tabular}[c]{@{}c@{}}Human\\ Appearance\end{tabular} & Appearance1   & Appearance2   & Appearance3   & Appearance4   \\
TSN                                                        & 0.19 / 67.41  & 0.46 / 84.26  & 7.31 / 87.04  & 15.09 / 88.06 \\
I3D                                                        & 48.61 / 81.48 & 72.50 / 88.80 & 70.83 / 84.44 & 61.39 / 81.11 \\
\begin{tabular}[c]{@{}c@{}}Human\\ Appearance\end{tabular} & Appearance5   & Appearance6   & Appearance7   & Appearance8   \\
TSN                                                        & 48.06 / 78.70 & 39.91 / 79.81 & 16.20 / 64.07 & 11.57 / 79.07 \\
I3D                                                        & 51.11 / 87.69 & 61.20 / 87.69 & 23.24 / 57.50 & 48.89 / 79.91
\end{tabular}
\caption{Classifying accuracy of both TSN and I3D is influenced by human appearance. Take Push-ups as an example, TSN and I3D were tested on the aggregation of Push-ups azimuth split, elevation split and distance split over 8 distinct human appearances. 
\label{tab:appearance}}
\end{table*}


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/Figure6.png}
    \caption{Similar trend emerges from Push-ups azimuth score curves yielded by TSN corresponding to 8 distinct synthetic human appearances. }
    \label{fig:azimuth}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figure/Figure7.png}
    \caption{Classification scores for real human Push-ups videos follow the same trend obtained from synthetic human Push-ups videos.}
    \label{fig:real_verify}
\end{figure}




==> note/4_exp_outline.tex <==

4.1 Image-space transform
1. 引出两种transform, image-processing 和semantic transform
4.1.1. image-processing transform
1. image-processing transform includes 是怎么实现的
2. 实验得出的数据是什么样的
3. 简单的变换发现模型不robust的，有很大的降低，counter-intuitive.
4.1.2 semantic transform.
1. 使用Mask\_RCNN 将Input分为前景和背景，怎么计算准确率的变化。
2. 在UCF101上的结果显著地分成三类，分别是什么样子的，说明了model如何。 
3. 好的模型是CR_f，CR_b == 0，但大部分类型都不满足这个要求
3. 我们的方法能够发现有些类型是只用背景而不是前景来判断的。 由于前景和背景都包含了Human pose & shape, 好model应该根据背景和前景都能推理Human motion,准确分类。 但是出现了CRfCRb的分化，说明model是通过检测图片里面的texture, object来分类Human activity的，它没有用到Human motion。
4. 对于有object的物体，物体在背景， 背景准确率高， 物体在前景，前景准确率高，说明model需通过检测物体来分类。
5. 对于定量的结果，我们使用CAM来寻找空间上的解释。

4.2 3D transform
 我们的synthetic数据来自哪里，这些synthetic video是怎么造出来的。

3. 记录了score， score显示TSN和i3d对viewpoint视sensitive的，但是sensitive的程度，sensitive额pattern取决于model, activity class和factor。
4. 如果一个Model对于某一个activity class的某一个viewpoint factor非常敏感，出现了明显的react pattern, 我们可以进一步可视化Model的intermediate feature. 
6.对于一些factor, model在不同的appearance上有不同的score curve，对另外一些factor，model在所有appearance上给出的是曲线是非常相近的。
7. 如果我们在real data里面控制这些不同synthetic appearance都给出相同趋势的factor，仍用同一个Model在realdata 上检测，出来的趋势也是一样的。
8. 3d transform可以告诉我么一个model对于一个factor的详细反应，而且在synthetic data上面得到的普遍性规律在real data里面依然成立。
